DiffMoE: Dynamic Token Selection for Scalable Diffusion Transformers

Diffusion models have demonstrated remarkable success in various image generation tasks, but their performance is often limited by the uniform processing of inputs across varying conditions and noise levels. To address this limitation, we propose a novel approach that leverages the inherent heterogeneity of the diffusion process. Our method, DiffMoE, introduces a batch-level global token pool that enables experts to access global token distributions during training, promoting specialized expert behavior. To unleash the full potential of the diffusion process, DiffMoE incorporates a capacity predictor that dynamically allocates computational resources based on noise levels and sample complexity. Through comprehensive evaluation, DiffMoE achieves state-of-the-art performance among diffusion models on ImageNet benchmark, substantially outperforming both dense architectures with 3x activated parameters and existing MoE approaches while maintaining 1x activated parameters. The effectiveness of our approach extends beyond class-conditional generation to more challenging tasks such as text-to-image generation, demonstrating its broad applicability across different diffusion model applications. Project Page: https://shiml20.github.io/DiffMoE/

==> cache.tex <==
Diffusion Transformers (DiTs) have emerged as the dominant architecture for visual generation tasks, yet their uniform processing of inputs across varying conditions and noise levels fails to leverage the inherent heterogeneity of the diffusion process. While recent mixture-of-experts (MoE) approaches attempt to address this limitation, they struggle to achieve significant improvements due to their restricted token accessibility and fixed computational patterns. We present **DiffMoE**, a novel MoE-based architecture that enables experts to access global token distributions through a **batch-level global token pool** during training, promoting specialized expert behavior. To unleash the full potential of inherent heterogeneity, DiffMoE incorporates a **capacity predictor** that dynamically allocates computational resources based on noise levels and sample complexity. Through comprehensive evaluation, DiffMoE achieves state-of-the-art performance among diffusion models on ImageNet benchmark, substantially outperforming both dense architectures with 1.5x activated parameters and existing MoE approaches while maintaining 1x activated parameters. The effectiveness of our approach extends beyond class-conditional generation to more challenging tasks such as text-to-image generation, demonstrating its broad applicability across different diffusion model applications.

